ACL-rlg: A Dataset for Reading List Generation

Familiarizing oneself with a new scientific field and its existing literature can be daunting due to the large amount of available articles. Curated lists of academic references, or reading lists, compiled by experts, offer a structured way to gain a comprehensive overview of a domain or a specific scientific challenge. In this work, we introduce ACL-rlg, the largest open expert-annotated reading list dataset. We also provide multiple baselines for evaluating reading list generation and formally define it as a retrieval task. Our qualitative study highlights the fact that traditional scholarly search engines and indexing methods perform poorly on this task, and GPT-4o, despite showing better results, exhibits signs of potential data contamination.

==> tables/datasets.tex <==
\begin{tabular}{l p{140pt} p{140pt} r r c c} 
\toprule
\textbf{Dataset} & \textbf{Data source} & \textbf{Domain} & \textbf{Lists no.} & \textbf{Items no.} & \textbf{Expert} & \textbf{Available} \\ 
\midrule

\citet{10.1145/1864708.1864740} & ACM Computing Surveys & Informatics & 220 & $\geq$15 & \xmark & \xmark \\

\citet{10.1109/JCDL.2019.00011} & Scopus (Reviews and Short Surveys) & Informatics, Engineering & 1~648 & Unk. & \xmark & \xmark \\

SurveyBank~\cite{9835398} & S2ORC, Google Scholar  & NLP, Machine Learning, Artificial intelligence, Deep learning, Information extraction & 9~321 & $\sim$58 & \xmark & \cmark \\

\midrule

\citet{UCAM-CL-TR-848} & ACL Anthology Network & NLP & 8 & $\sim$12 & \cmark & \cmark \\

\textbf{Our dataset} & ACL Anthology & NLP & 85 & $\sim$8 & \cmark & \cmark \\
\bottomrule
\end{tabular}%


==> tables/exp2.tex <==
\begin{tabular}{lrrr|rrr|rrr|rrr}
\toprule
 & \multicolumn{3}{c|}{\textbf{Semantic Scholar}} & \multicolumn{3}{c|}{\textbf{Google Scholar}} & \multicolumn{3}{c}{\textbf{GPT-4o (Avg. run)}} & \multicolumn{3}{c}{\textbf{Gemini (Avg. run)}} \\
 \cmidrule(lr){2-4} \cmidrule(lr){5-7}  \cmidrule(lr){8-10} \cmidrule(lr){11-13} 
 & recall & ndcg & mrr & recall & ndcg & mrr & recall & ndcg & mrr & recall & ndcg & mrr \\
\midrule
A1 (phd) & 5.3 & 3.6 & 6.2 & 8.4 & 7.2 & 13.0 & 11.3 & 11.2 & 21.5 & 2.7 & 2.5 & 4.9\\
A2 (postdoc) & 4.0 & 3.2 & 5.9 & 5.2 & 4.7 & 9.7 & 10.8 & 10.4 & 19.9 & 2.6 & 2.5 & 5.5\\
A3 (senior) & 6.6 & 4.7 & 8.4 & 8.8 & 7.1 & 12.7 & 12.4 & 12.8 & 25.4 & 2.8 & 2.5 & 5.1\\
\midrule
Mean & 5.3 & 3.8 & 6.8 & 7.5 & 6.4 & 11.8 & 11.5 & 11.4 & 22.3 & 2.7 & 2.5 & 5.2 \\
\bottomrule
\end{tabular}


==> tables/exp3.tex <==
\begin{tabular}{lrrr|rrr|rrr}
\toprule
 & \multicolumn{3}{c|}{\textbf{Semantic Scholar}} & \multicolumn{3}{c|}{\textbf{BM25}} & \multicolumn{3}{c}{\textbf{SPECTER2}} \\
  \cmidrule(lr){2-4} \cmidrule(lr){5-7}  \cmidrule(lr){8-10} 
 & recall & ndcg & mrr & recall & ndcg & mrr & recall & ndcg & mrr \\
\midrule
A1 (phd) & 8.4 & 5.5 & 7.6 & 8.9 & 5.7 & 8.8 & 5.8 & 3.1 & 3.3 \\
A2 (postdoc) & 6.7 & 5.5 & 8.2 & 9.2 & 5.5 & 6.3 & 5.7 & 3.4 & 4.6 \\
A3 (senior) & 9.5 & 7.2 & 11.0 & 11.2 & 6.6 & 9.2 & 8.2 & 4.7 & 5.8 \\
\midrule
Mean & 8.2 & 6.1 & 9.0 & 9.7 & 5.9 & 8.1 & 6.6 & 3.7 & 4.6 \\
\bottomrule
\end{tabular}

